Copula Flows for Synthetic Data Generation

The ability to generate high-fidelity synthetic data is crucial when available (real) data is limited or where privacy and data protection standards allow only for limited use of the given data, e.g., in medical and financial data-sets. Current state-of-the-art methods for synthetic data generation are based on generative models, such as Generative Adversarial Networks (GANs). Even though GANs have achieved remarkable results in synthetic data generation, they are often challenging to interpret.Furthermore, GAN-based methods can suffer when used with mixed real and categorical variables.Moreover, loss function (discriminator loss) design itself is problem specific, i.e., the generative model may not be useful for tasks it was not explicitly trained for. In this paper, we propose to use a probabilistic model as a synthetic data generator. Learning the probabilistic model for the data is equivalent to estimating the density of the data. Based on the copula theory, we divide the density estimation task into two parts, i.e., estimating univariate marginals and estimating the multivariate copula density over the univariate marginals. We use normalising flows to learn both the copula density and univariate marginals. We benchmark our method on both simulated and real data-sets in terms of density estimation as well as the ability to generate high-fidelity synthetic data

==> 9_extra_text.tex <==
\section{Comparing Generative Samples}
We need to clearly define what the metric we are comparing against. This is
simple question of saying if we think our method is better then we need to
clearly have a valid metric. 

candidates so far, really overweight on kernel based methods
\begin{itemize}
    \item Log-likelihood of test data, we have full probabilistic model, can't
    directly compare with GAN based papers. 
    \item Maximum Mean Discrepancy MMD
    \item Omptised Kernel version of MMD ( Generative Models and Model Criticism
via Optimized Maximum Mean Discrepancy (2017))
    \item two-sample classifier tests (Gretton, Borgwardt, Rasch, Schölkopf,
    Smola. A kernel two-sample test (2012))
    \item Goodness of fit test, Finite sample Stien Discrepency [FSSD, NeurIPS
    2017 Best Paper], alternative to log-likelihood. 
\end{itemize}

\section{Main Method}
Crux of the paper
\begin{itemize}
	\item Learn copula based models to learn joint densities correctly.This
	method separates joint density learning and marginal density learning.
	copula learns joint and marginals are 1d densities which are easy to learn
	\item we can learn arbitrarily complex marginal densities, using normalising
	flows [cite(renzende, shakir icml 2015)].
	\item normalising flows relies on give us invertible function
	transformations, which can use to get uniform marginals [vias CDF of base
	distribution like univariate Gaussian for example ]
	\item Use Masked auto-regressive flows to learn the joint density of the
	uniform marginals (which is a copula density, assuming it exists) 
	\item to generate a sample from the model, first sample from copula to
	obtain correlated uniform random variables and then push through the learned
	normalising flow map
\end{itemize}


Normalizing flows transform a probability distribution using an invertible
function (Tabak and Turner, 2013; Rezende and Mohamed, 2015; Rippel and Adams,
2013).


For multivariate case we can readily extend the  transform as well as the
inverse quantile function or flow $ \mathcal{F} $. Let $ \vec X = {X_1, \ldots,
X_d} $ be a random vector with distribution function $ F $. Let the vector $
\vec U= {U_1, \ldots, U_d}$ be iid $ \uniform{1} $ distributed random variable
then the multivariate quantile transform $ Y :=  \tau\inv (V) $ can be defined
recursively as, 
\begin{align}
Y1 &:= F_{1}\inv (U_1) \\
Y_k &:= F\inv_{k|1, \ldots k-1}\left( U_k | Y_1, \ldots, Y_{k-1} \right),  \quad 2 \leq k \leq d \nonumber
\end{align}, 
where $ F\inv_{k|1, \ldots k-1} $ denotes conditional distribution function. 


We can apply nomalizing flow methods to learn the conditional distribution
function $  F_{k|1, \ldots k-1} $. This is presented as autoregressive density
estimation in Masked Autoregressive Flows MAF~\cite{Papamakarios2017}. 




we have parametric models for the marginal densities $f_{X_i}(x_i | \vec
\theta_i)$ where $ \vec \theta_i $ are parameters of the $ i^th $ marginal. And
the joint copula density $\vec c_{\mat X}( \vec x)$ is defined by $\vec
\theta_c$ the log-likelihood for data set $\mat D = (\vec x^{(1)}, \ldots, \vec
x^{(N)})$can be written as, 
\begin{align}
\log \mathcal{L} &(\mat D | \vec \theta_1, \vec  \ldots, \vec \theta_d, \vec \theta_c)  \\ &= \log \vec f_{\mat X}(\vec x) \\
&=  \log c_{\mat X}\left (F_{X_1}(x_1), \ldots, F_{X_d}(x_d) | \vec \theta_c \right) \nonumber \\
& \quad \quad + \sum_{i}^{d}\log \left(  f_{X_i}(x_i | \vec \theta_i)  \right) 
\end{align}



We can then train the model with gradient decent, as the likelihood function
separable in data points we can do minibatching/ stochastic gradient descent. 




%%%%%%\######################### BackGround Tex 


\subsection{Normalising Flows }

Normalising flows~\cite{Rezende2015} construct an invertible flow function, e.g.
$G$,  that transforms one density into another density. An alternative way to
look at flow densities is the classical way of generating samples of random
variable $ X $ following a distribution function $ F $. A standard way to
genrate randomvariable is 



that we  can learn distribution functions $ F_{X}(x)  $ needed for training
copulas via normalising flow function. 

\textbf{rember to write about generating truncated distributions, e.g., truncated normal, no rejection sampling is needed if know inverse CDF }

\begin{theorem}
	\label{thm:copulaInvariance}
	Let X and Y be continuous random variables with copula $ C_{XY} $. If $
	\alpha $ and $\beta  $ are strictly increasing on $ \range X $ and$ \range Y
	$, respectively, then the copula $ C_{ \alpha (X) \, \beta(Y)}= C_{XY} $,
	i.e., $ C_{XY} $ is invariant under strictly increasing transofrmations of $
	X $ and $ Y $
\end{theorem}
proof see appendix or \cite{Nelson}


%\section{Copulas}


\subsubsection{Hoeffding and Frechet bounds}
%  Do we need or use this ? if not no need to mentions them 


\subsubsection{Training Copulas}
%
%The function $  G$ can be referred to as flow and it can implemented as series
% non-linear transofmr to learn complex functions. Let x be a D-dimensional
% continuous random variable whose density can be computed efficiently. Given an
% invertible function $f: \mathbb{R}^{D} \rightarrow \mathbb{R}^{D}$, the
% change-of-variables formula provides an explicit construction of the induced
% distribution on the function’s output, y = f(x):
%
%
%
%The transformation f is referred to as a flow and p(x) is referred to as the
%base distribution. Composing multiple flows can induce further complex
%distributions that increase the expressivity of p(y)

The bottle neck is the Jacobian computation $ \left(\partial G^{-1} / \partial
x\right) $ in \ref{eq:normFlow} which is of order $O (D^3)$ for D dimensional
map . So the main aim of recent developments in normalising flow based methods
is to create flow maps where  Jacobain is easier to compute. This is typically
true for functions with lower triangular Jacobians [\textit{May be explain this
bti more}]. Masked Autoregressive flows \cite{Papamakarios2017}

%\subsection{Normalising Flows and Copulas } Show how multivariate Gaussian
% Copula is is essentially a generative map X -> AX -> CDF() -> Multivariate
% Gaussian Copula


\subsection{Masked Autoregressive Flows}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We can express the density $\vec f_{\mat X}(\vec x)$ as production of
autoregressive dependence, i.e., $\vec f_{\mat X}(\vec x) = \prod_i f_{X_i}(x_i
| x_{1:i-1})$. We can model this by building flow maps recursively, i.e., $
F_{X}(\vec x) = F_{X_d} \left( \ldots F_{X_2}(F_{X_1}(x_1))) \right)$. Normally,
each individual densities are expressed in terms of lcation scale family, for
example normal distribution as, 
\begin{align}
f_{X_i}\left(x_{i} | \mathbf{x}_{1: i-1}\right) &=\mathcal{N}\left(x_{i} | \mu_{i},\left(\exp \alpha_{i}\right)^{2}\right) 
\end{align}
Due to autoregressive construction Jacobian is lower triangular, hence,
determinant of Jacobian is just $\exp \left(-\sum_i \alpha_{i}\right)$, where
$\alpha_{i} = g_{NN}(\vec x_{1:i-1})$ see ~\cite{Papamakarios2017} more details.


The neural networks function can be conveniently compute by masking specifi
weights to impose recursive nature.  one such example is
MADE~\cite{Germain2015}. Important advantage of using MADE is that flow can be
implemented in one forward pass rather than recursive construction. Masked
autoregressive flows MAF~\cite{Papamakarios2017} is made by stacking MADE layers
one after the other.  For better performance one can also permute data so that
the autoregressive network can be more expressive. permutation is invertible
rotation map with unity determinant can improve performance of MAFs.


this is expressed as a combination of Gaussian densities. We can express this in
terms of inverse of distribution function 

\begin{align}
F_{X_{d+1}}^{-1}(x_{d+1}) = \frac{x_{d+1}- \mu_{X_{1:d}}}{\sigma_{X_{1:d}}} 
\end{align}


\subsection{Spline Flows}

Another alternative to implement invertible maps with lower triangular Jacobians
is coupling transform [Cite NICE and Real NVP paper]. In neural spline flows the
coupling is implemented by monotonic rational quadratic transforms [Cite neural
spline and original spline paper]

The spline maps an interval [-B, B] to [-B, B] using K different
rational-quadratic fucntions set at knots $\lbrace \left( x^k,
y^k\right)\rbrace$ where $k= 0, \ldots, K$ .  the spline can be made
monotonically increasing function by placeing knots monotonically increasing
fashion between the $ (-B, B) $ to $ (B, B) $. 

Do we need to expand it here or when we actually introduce changes to the basic
model ?

Cone to complete this based on next secion 

\begin{itemize}
	\item [1.]  A 
\end{itemize}


\sanket {need to think and rephrase next 2 paras keeping the gist}


An interesting question to ask what is distribution function of the univariate
marginals $ U_{X}, U_{Y} $ obtained by probability integral transform of  $ X, Y
$ via distributions, i.e.,  $ U_X = F_X (x) , \, \,  U_Y = F_Y (y) $. This
question is the primary motivation for study of copulas by Frechet [Cite
Frechet] and later consolidated by Sklar~\parencite{Sklar1959}.  

For synthetic data generation this question is crucial. Especially in privacy
preservation, where we perturb the data samples by another random process, this
changes the distribution function of the underlying variables, whereas for
synthetic data to be useful the relationships between the variables should be
preserved. This can be achieved by using copulas, 

We can do structure learning and build dependency graph, C, D or R-VIne copulas
as well as CBN are part of this we use stacked MAFs to automate this but ither
setting is plausible under the framework. 

make tree structure to MADE connection, with learned MADE we can do this in one
pass 

Show how multivariate Gaussian Copula is is essentially a generative map $ u
\rightarrow \phi(x) \rightarrow AX \rightarrow \phi(x)  $

